Enabling Cooperative IoT Security via Software Defined Networks (SDN)

Internet of Things (IoT) is becoming an increasingly attractive target for cybercriminals. We observe that many attacks to IoTs are launched in a collusive way, such as brute-force hacking usernames and passwords, to target at a particular victim. However, most of the time our defending mechanisms to such kind of attacks are carried out individually and independently, which leads to ineffective and weak defense. To this end, we propose to leverage Software Defined Networks (SDN) to enable cooperative security for legacy IP-based IoT devices. SDN decouples control plane and data plane, and can help bridge the knowledge divided between the application and network layers. In this paper, we discuss the IoT security problems and challenges, and present an SDN-based architecture to enable IoT security in a cooperative manner. Furthermore, we implemented a platform that can quickly share the attacking information with peer controllers and block the attacks. We carried out our experiments in both virtual and physical SDN environments with OpenFlow switches. Our evaluation results show that both environments can scale well to handle attacks, but hardware implementation is much more efficient than a virtual one.

==> Makefile <==
PRJ = aggregate

# to use eps figures
DVIOPT = -P cmz -t letter -G0

all : viewpdf 

#${PRJ}.dvi : *.tex *.bib 
#	pdflatex ${PRJ}; bibtex ${PRJ}; pdflatex ${PRJ}; pdflatex ${PRJ} 
#
#${PRJ}.ps : ${PRJ}.dvi
#	dvips ${DVIOPT} -o ${PRJ}.ps ${PRJ}.dvi

#${PRJ}.pdf : ${PRJ}.ps
${PRJ}.pdf : *.tex *.bib 
	pdflatex ${PRJ}; bibtex ${PRJ}; pdflatex ${PRJ}; pdflatex ${PRJ} 
#	ps2pdf ${PRJ}.ps ${PRJ}.pdf

dvi : ${PRJ}.dvi

ps : ${PRJ}.ps

pdf : ${PRJ}.pdf

viewdvi : ${PRJ}.dvi
	xdvi ${PRJ}.dvi &

viewps : ${PRJ}.ps
	open ${PRJ}.ps &

viewpdf : ${PRJ}.pdf
	open ${PRJ}.pdf &

# to use non-eps figures.
#all : view 

#${PRJ}.pdf : *.tex 
#	pdflatex ${PRJ}; bibtex ${PRJ}; pdflatex ${PRJ}; pdflatex ${PRJ}

#pdf: ${PRJ}.pdf

#view : ${PRJ}.pdf
#	open ${PRJ}.pdf &

pack : pdf
	/bin/rm -f ../${PRJ}.tgz; tar -zcf ../${PRJ}.tgz Makefile *.tex IEEEtran.cls net.bib ${PRJ}.pdf figure 

clean:
	/bin/rm -f *.toc *.aux *.bbl *.blg *.log *.dvi *~* *.bak ${PRJ}.pdf ${PRJ}.ps

distclean:
	/bin/rm -f *.toc *.aux *.bbl *.blg *.log ${PRJ}.dvi ${PRJ}.ps ${PRJ}.pdf *~* *.bak

#cut : ${PRJ}.dvi 
#	dvips -t letter -o summary.ps -p=2 -l=2 ${PRJ}.dvi
#	ps2pdf summary.ps summary.pdf
#	/bin/rm summary.ps \
#
#	dvips -t letter -o description.ps -p=3 -l=17 ${PRJ}.dvi
#	ps2pdf description.ps description.pdf
#	/bin/rm description.ps \
#
#	dvips -t letter -o references.ps -p=18 -l=20 ${PRJ}.dvi
#	ps2pdf references.ps references.pdf
#	/bin/rm references.ps



==> aggregation.tex <==
\section{adding route aggregation to quagga}
\label{sec:aggregation}
%
%   - background: some background on quagga (the figure showing Quagga's workflow and some explanation)
%     - challenges: not just listing the three challenges, but also how we solved each of them in one or two sentences (please be specific, not vague as I mentioned above)
%     - design: a figure showing the updated workflow and some explanation of the updated workflow
%     - module implementation: explain each module's implementation in some detail
%     
The first objective of our work is to add FIB aggregation and performance monitoring to Quagga without major code changes and negative performance impact.  This ensures that we do not inadvertently change Quagga's implementation logic and that our new features do not slow down the core routing and forwarding functionality.   These considerations led to the updated Quagga system, as depicted in Figure~\ref{fig:quagga_aa}.

\begin{figure}
\begin{center}
     \includegraphics[width=2.8in]{figures/Quagga.pdf}
\caption{\label{fig:quagga_aa}Quagga Modules with FIB Aggregation}
\end{center}
\vspace{-8mm}
\end{figure}


%\subsection{Quagga Background}

\subsection{FIB Aggregation}
\label{sec:quagga_design}

In order to aggregate the FIB without changing Quagga significantly,  we keep our FIB aggregation code out of the existing Quagga code.  We add an Interception Module to intercept every FIB update after it is received by the Zebra daemon and pass them to the FIB Aggregation Module (Figure~\ref{fig:quagga_aa}).  Once the Interception Module receives the aggregated FIB changes back from the FIB Aggregation module, it applies them to the Kernel FIB.   Below we describe these two modules in detail.

The Interception Module's major functionality includes fetching static routes, interception of inbound FIB updates, application of aggregated FIB updates to the Kernel FIB, and logging.  The FIB updates fall into two categories: (a) \emph{Route Installs}: adding one or more entries from the FIB for a new address prefix; and (b) \emph{Route Uninstalls}: deleting one or more entries from the FIB for an existing address prefix.   

%TODO: need more detail on aggregation module
The Aggregation Module interacts directly with the Interception Module but not with other parts of Quagga.  It houses some temporary data structures that are needed to perform effective and incremental table aggregation.  It currently encapsulates the logic of our FIFA-S  algorithm~\cite{Liu13:FIFA} which can be easily replaced with any other FIB aggregation algorithm.   Below we highlight several implementation issues that we did not encounter in our previous stand-alone implementation.

%TODO: need better explanation of the following issues.  They are very vague.
\begin{itemize}

\item \emph{Processing Static Routes}: when we plugged in the Aggregation Module to Quagga, we found a few duplicate route prefixes with different next-hop values.  It turned out that static routes were pre-configured during Quagga's start-up. Our solution is to introduce these static routes into the aggregation module but do not aggregate them.  More specifically, we set particular flags for these routes so that they will not be aggregated with other routes. 

\item \emph{Updating Kernel FIB}: without aggregation, one route change will generate one Kernel FIB change. With aggregation, however, one route change may lead to zero or more FIB changes because we have to remove redundant routes from FIB to keep it compressed all the time.   We also learned an important fact that an update with a next-hop value change actually consists of two FIB operations -- Quagga first withdraws the prefix with the old next-hop value and then injects the same prefix with a new next-hop value. 

\item \emph{Handling Recursive Next-hop}: The FIB entries propagated inside Quagga sometimes have next-hops that are "recursive" in nature. This means the next-hop to reach a destination does not refer to a direct neighbor but to another intermediate node that lies on the path to the destination.  For example, the recursive next-hop could be the iBGP neighbor that is closest to the destination (among all the iBGP neighbors of the node), but may be several IP hops away from this router.  It is therefore necessary to look up the address of the recursive next-hop in the FIB (one or more times) until we resolve this recursive next-hop to a directly connected next-hop neighbor. We did not realize the usage of recursive next-hop in Quagga initially and had difficulty understanding why the aggregated FIB is incorrect in some cases. In fact, the Quagga route data structure includes a recursive next-hop flag to determine which data field (regular next-hop or recursive next-hop) to use for the next-hop value. Since our aggregation module originally accepts and returns only non-recursive next-hop values, we had to modify our process to handle such recursive updates.

\end{itemize}

\subsection{Performance Monitoring}

When adding FIB aggregation to a routing software, we expect the changes to result in as little CPU overhead as possible and at the same time improve other performance metrics such as memory usage.  The impact of our changes can only be quantified through low level  performance metrics captured at runtime. Some metrics pertain to the overall Quagga system performance such as CPU usage and routing process' virtual memory usage.  Other metrics are specific to FIB aggregation such as FIB entry count, FIB memory usage, and number of updates made to the FIB. 

The primary statistics captured by the Performance Monitoring module include (a) CPU and virtual memory usage of the OS, BGP daemon and Zebra daemon; (b) Kernel FIB's memory usage; (c) Kernel FIB entry count; (d) number of Route Installs and Route Uninstalls intercepted and actually performed.   Part of the module is implemented within the Zebra daemon to support capturing of statistics on Zebra's updates to the Kernel FIB.

We capture the memory and CPU utilization metrics through periodic operations on the files that the Unix kernel maintains in its proc directory. 
%CPU usages are recorded in terms of multiple clock cycle values which are periodically updated in system process files. These process files also store virtual and actual memory utilizations in appropriate memory units. 
Similarly, some metrics related to the Kernel's FIB are computed from the internal kernel file /proc/net/route which holds the Kernel's FIB.  In addition, we capture routing update statistics in terms of Route Installs and Route Uninstalls by the addition of some program variables within the Zebra daemon. All the information gathered by the monitoring application is made available through command line options and log files.

%With these new additions at each network node and the basic topology creation mechanism explained earlier, we were able to create a virtual network capable of running any combination of network protocols and routing table aggregation at every node. It was therefore possible to create a working model of a real-world network architecture and access its performance metrics at every node level for any required network configuration.



==> bg.tex <==
\section{Background}
\subsection{Route caching}
Traditional architecture of a router implies two main components, the \textbf{control plane} responsible for collecting and distributing routes, and the \textbf{data plane} with the Forwarding Information Base (FIB). The data plane is responsible for forwarding packets. To ensure fast Longest Prefix Match (LPM) lookup in FIB, hardware manufactures build the data plane with TCAM-based forwarding engines. 

The drawback of using TCAM is that TCAM is highly energy consumptive. The situation is aggravated by the fact that the size of the FIB is constantly growing, pressing network operator to upgrade their legacy TCAM chips with newer, even more energy demanding models. However, due to the fact that not all of the entries in a FIB are equally popular among end users[cite? graphs?], in an alternative router architecture, the least popular entries can be moved to the slower SRAM and DRAM chips with cheap and less energy demanding memory. The approach is known in academia as $Route$ $Caching$. When designing an architecture of a router with separate routing tables (on high and slow speed memory units) it is important to consider the following aspects: (1) Cache miss ratio must be minimized and be close to 0\%; (2) Cache miss entries must not cause queues at a slow memory's buffers with consequent packet drops; (3) Cache miss latencies must be reasonable; (4) Cache replacement operations must be processed efficiently without high computational overhead; (5) a problem known as $cache$ $hiding$ must be avoided in order to guarantee correct forwarding. Below we give the description of the $cache$ $hiding$.

$Cache$ $hiding$  is a natural problem that comes from dropping entries from a routing table that uses the $Longest$ $Prefix$ $Match$ ($LPM$) rule to find a match for an IP address. Specifically, suppose the full FIB contains a more specific prefix $p_{A} = 128.153.64.0/18$ than a prefix $p_{B} = 128.153.0.0/16$ existing in a cache. The next hop assigned to $p_{A}$ in the full FIB is $A$, while IP packets with addresses matching $p_{B}$ are forwarded to a next hop $B$. In such case, a packet with IP destination address $128.153.183.226$ matching $p_{A}$ will be forwarded to the next hop $B$ rather than $A$, since in the cached FIB its Longest Prefix Match is the prefix $p_{B}$. $Cache$ $hiding$ may be caused by (1) incorrect initial cache with less specific prefixes than in the full FIB on the slow memory; (2) After BGP prefix announcement, when a more specific prefix that a one existing in the cache is installed into the full FIB; (3) Similarly, BGP withdrawal might cause a situation when a cache contains less specific entries than in the full FIB.

\subsection{Programmable Data Plane}
Software-Defined Networking implementations such as OpenFlow[cite] are highly useful for building programmable networks. However, constrains in the data plane limit the ways a packet might be parsed and processed in the data plane. P4[cite], a high-level language for programming protocol-independent packet processors, represents a model for the future era of the switches with the programmable data plane. P4-switches are supposed to have a programmable packet parser as well as programmable ingress and egress pipelines. This gives network engineers opportunity to program a switch with ability to process packets of any protocol, define multiple match-action tables through which the network flow must go, clone packets and recirculate them in the switch. P4 also generates API for the control plane for managing match-action tables. P4 introduces the concept of a packet metadata, when each packet processed by the switch is accompanied with data through ingress and egress pipeline. P4-switch is supposed to have a number of registers available for calculations inside the data plane. P4 enables hashing base and the set of metadata fields or packet headers.

==> simulation.tex <==
\section{Emulating an ISP network}
\label{sec:simulation}

The second objective of our work is to set up a \emph{realistic network environment} to demonstrate the performance of our FIB aggregation algorithm.  To this end, we use VirtualBox, BGPSimple, and real ISPs' routing data to emulate a real operational network.  Note that our methodology can be used to emulate any network, but in this section, we use the Internet2 Abilene topology as an example to illustrate our methodology.  

\begin{figure}[tb]
\begin{center}
     \includegraphics[width=2.5in]{figures/topology}
\caption{\label{fig:topology}Virtual Network Setup}
\end{center}
\vspace{-8mm}
\end{figure}

Figure~\ref{fig:topology} shows our virtual network, which includes a total of 9 routers in the Internet2 topology and 9 external BGP speakers belonging to other ISPs that exchange routing information with Internet2.  Each node is on a separate virtual machine.    Each Internet2 router runs either the original Quagga or our updated version of Quagga (specifically the Zebra, OSPF, and BGP daemons).  Each BGP speaker runs the BGPSimple program that sends real routing updates to the BGP peer. 

%TODO: do we run OSPFN on the BGP speaker nodes?
We use OSPF to establish intra-domain connectivity among all of the Internet2 nodes.
%which results in route additions to the Kernel FIB for complete intra-domain connectivity. 
The BGP daemons on each Internet2 node then use this base connectivity to establish BGP peering session with their iBGP peers.  For  simplicity, we use full-mesh iBGP peering, i.e., every router has an iBGP session with every other router in the same network.  For a larger topology, we can use Route Reflectors to reduce the number of iBGP sessions.

In order to attain equivalence between the virtual network and a real world ISP, we need the presence of the huge volume of BGP routing updates in the Internet.  Fortunately, BGP routing table and updates from many ISPs are being collected by a number of projects.  
%This is done through tabledump and update �les which are organized chronologically for a lot of actual internet router pre�xes. These �les include snapshots of routing tables of BGP routers in the internet formatted in the form of route announcements and withdrawals. 
We use the BGP data from the RouterViews project of the University of Oregon~\cite{routeviews} and the BGPMon project of Colorado State University~\cite{BGPmon}. The RouterViews project provides BGP table dumps and update files archived at regular intervals while the BGPMon project provides \emph{live} BGP updates in addition to archived BGP data. 
%These are two among the many freely available data sources which make BGP routing information available and it is possible to use these �les as feeds for BGP speaker applications.

%A real-world routing network transits frequent and consistent volume of network control traf�c in order to maintain end-to-end connectivity between its nodes. The control updates format and handshake mechanisms vary depending on the routing protocol being followed. But these updates, although not constituting the majority of the network traf�c, form a signi�cant part as they control the forwarding information held in the routing tables and thereby the overall routing process. The next section details how we add real-world routing updates to our experimental setup.

%We can make a virtual network equivalent to a real-world routing architecture if we need to simulate a very similar level of control traffic. This requires the infusion and propagation of an equivalent volume of protocol speci�c updates which get processed by the individual routing nodes and cause updates to the routing tables. For the purpose of this paper and our research we will focus the control traf�c speci�c to only the BGP protocol. 

We modified the BGPSimple program to pump the BGP data into the network.  The program first reads a routing table from a BGP table dump file (from RouteViews or BGPMon) and then sends the resulting BGP updates over its BGP session so that the peer can establish an initial BGP table.  Since there are hundreds of thousands of entries in a full routing table, we added pacing to the BGPSimple program  so that the peer does not become overwhelmed by the initial influx of updates.  The program then sends subsequent BGP updates as they become available.  These updates are obtained from either the BGP update files downloaded from RouteViews or a live stream of BGP updates from BGPMon.  
%The BGP speaker can also filter BGP updates based on many parameters such as originating peer and address prefix being advertised. 
%These updates are spoken in the form of BGP announcements and withdrawals which when reach the connected routers, are processed and propagated to other BGP peers in the network. In other words, the BGP feed provided to the speaker in a way determine the control traffic moving around in the network. Therefore to make a node on our virtual network function in a similar to an actual BGP router only required feeding routing updates as processed by latter.
In order to evaluate the performance of our system under high routing load, we used large routing tables with 450,000 prefixes on average. 
%The speakers were also configured to switch over to live BGP update channel of Colorado State once they finish processing their initial tabledump files.



%As each node of the Abilene network represents a separate BGP router having its own volume of peering update channel, we added a total of 9 BGP Speaker nodes (ones speaker for each virtual router node) to our setup. Each of these speakers were con�gured for processing a BGP tabledump �le collected for a recent date from the data sources corresponding to an actual internet BGP router. 
